Vacuum Energy in Modern Cosmology: an analysis of quantum field theory in curved spaces and its application to cosmological spacetimes

The last decades have witnessed an unprecedented advancement in our knowledge of the large scale universe. In particular, increasingly accurate cosmological observations have allowed us to discover a form of "dark energy", which presently dominates the expansion of the universe. On the other hand, fundamental problems in the standard cosmological model point towards the possibility of a primordial inflationary period. Both these expansion phases have in common the fact that they should be governed by forms of energy with properties much similar to those of vacuum energy of classical or quantum fields. In the meanwhile, quantum field theory in curved spaces (QFTCS) has proved a rich framework to analyze phenomena of a quantum nature in regimes where spacetime curvature is relevant, but not too extreme; particularly, it yields novel insights on the structure and dynamics of quantum vacuum. In this dissertation, we make a thorough exposition of the fundamentals of QFTCS and present some of its applications in cosmological spacetimes. Particular attention is given to the construction of an empirical notion of particles through an idealized model of particle detectors, and to the phenomenon of particle creation in expanding FLRW spacetimes. Further, we develop the procedure of adiabatic renormalization, and use it to compute the renormalized stress tensor in these spacetimes. For a noninteracting scalar field in de Sitter spaces, we find that it takes the form of a cosmological constant, although a quantitatively self-consistent value with the background expansion can only be found at Planckian densities. We also present a construction of a simple inflationary model, driven by a self-interacting classical scalar field, and show how the quantized fluctuations of this field could give rise to a nearly scale-invariant power spectrum, like the one that is currently observed in the CMB.

==> USPSC-fichacatalografica.tex <==
% ---
% Inserir a ficha bibliografica
% ---
% Isto é um exemplo de Ficha Catalográfica, ou ``Dados internacionais de
% catalogação-na-publicação''. Você pode utilizar este modelo como referência. 
% Porém, provavelmente a biblioteca da sua universidade lhe fornecerá um PDF
% com a ficha catalográfica definitiva após a defesa do trabalho. Quando estiver
% com o documento, salve-o como PDF no diretório do seu projeto e substitua todo
% o conteúdo de implementação deste arquivo pelo comando abaixo:
%
\begin{fichacatalografica}
	\hspace{-1.4cm}
	\imprimirnotaautorizacao \\ \\
	%\sffamily
	\vspace*{\fill}					% Posição vertical
	\begin{center}					% Minipage Centralizado
		\imprimirnotabib \\
\begin{table}[htb]
	\scriptsize
	\centering	
	\begin{tabular}{|p{0.9cm} p{8.7cm}|}
		\hline
	      & \\
		  &	  \imprimirautorficha     \\
		
		 \imprimircutter & 
							\hspace{0.4cm}\imprimirtitulo~  / ~\imprimirautor~ ;  ~\imprimirorientadorcorpoficha. -- 	\imprimirlocal, \imprimirdata.   \\
		
		  &  % Para incluir nota referente à versão corrigida no corpo da ficha,
			  % incluir % no início da linha acima e tirar a % do início da linha abaixo
			  %	\hspace{0.4cm} \imprimirtitulo~  / ~\imprimirautor~ ; ~\imprimirorientadorcorpoficha~- ~\imprimirnotafolharosto. -- \imprimirlocal, \imprimirdata.  \\
		
			\hspace{0.4cm}\pageref{LastPage} p.  \\ 
		  & \\
		  & 
		    \hspace{0.4cm}\imprimirnotaficha ~--~ 
						  \imprimirunidademin, 
						  \imprimiruniversidademin, 
		                  \imprimirdata. \\ 
		  & \\                 
		   % Para incluir nota referente à versão corrigida em notas,
		    % incluir uma % no início da linha acima e	
		    % tirar a % do início da linha abaixo
		    % & \hspace{0.4cm}\imprimirnotafolharosto \\ 
		  & \\ 
		  & \hspace{0.4cm}1. Stochastic. 2. Modulação acusto-óptica. 3. Potenciais ópticos dinâmicos. I. \imprimirorientadorficha. 
		   II. Título. \\
	
		     %Se houver co-orientador, inclua % antes da linha (antes de II. Título.) 
		     %          e tire a % antes do comando abaixo 
		     %III. Título. \\   
		  \hline
	\end{tabular}
\end{table}
	\end{center}
\end{fichacatalografica}
% ---



==> USPSC-pre-textual-IFSC.tex <==
%% USPSC-pre-textual-IFSC.tex
%% Camandos para defini��o do tipo de documento (tese ou disserta��o), %%�rea de concentra��o, op��o, pre�mbulo, titula��o 
%% referentes ao Programa de P�s-Gradua��o o IFSC
\instituicao{Instituto de F\'isica de S\~ao Carlos, Universidade de S\~ao Paulo}
\unidade{INSTITUTO DE F\'ISICA DE S\~AO CARLOS}
\unidademin{Instituto de F\'isica de S\~ao Carlos}
\universidademin{Universidade de S\~ao Paulo}

%\notafolharosto{Vers\~ao original}
%\notafolharosto{Original version} 

%\notafolharosto{Vers\~ao corrigida \\(Vers\~ao original dispon\'ivel na Unidade que aloja o Programa)}
\notafolharosto{Corrected version \\(Original version available on the Program Unit)}

%\notafolharosto{Versão original}

% ---
% dados complementares para CAPA e FOLHA DE ROSTO
% ---
\universidade{UNIVERSIDADE DE SÃO PAULO}
\titulo{Vacuum energy in modern cosmology: an analysis of quantum field theory in curved spaces and its application to cosmological spacetimes}
\titleabstract{Vacuum energy in modern cosmology: \textnormal{an analysis of quantum field theory in curved spaces and its application to cosmological spacetimes}}
%\tipotrabalho{{Estudos no diamante para aplica\c{c}\~oes em Tecnologias %Qu\^anticas.}
\autor{Eduardo Am\^ancio Barbosa Oliveira}
\autorficha{Oliveira, Eduardo A. B.}
\autorabr{OLIVEIRA, E. A. B.}

\cutter{S856m}
% Para gerar a ficha catalogr�fica sem o C�digo Cutter, basta 
% incluir uma % na linha acima e tirar a % da linha abaixo
%\cutter{ }

\local{S\~ao Carlos}
\data{2022}
% Quando for Orientador, basta incluir uma % antes do comando abaixo
\renewcommand{\orientadorname}{Orientador:}
% Quando for Coorientadora, basta tirar a % utilizar o comando abaixo
%\newcommand{\coorientadorname}{Coorientador:}
\orientador{Prof. Daniel Augusto Turolla Vanzella}
\orientadorcorpoficha{orientador Daniel Augusto Turolla Vanzella}
\orientadorficha{Vanzella, Daniel Augusto Turolla, orient}
%Se houver co-orientador, inclua % antes das duas linhas (antes dos comandos \orientadorcorpoficha e \orientadorficha) 
%          e tire a % antes dos 3 comandos abaixo
%\coorientador{Prof. Dr. Jo\~ao Alves Serqueira}
%\orientadorcorpoficha{orientadora Elisa Gon\c{c}alves Rodrigues ;  co-orientador Jo\~ao Alves Serqueira}
%\orientadorficha{Rodrigues, Elisa Gon\c{c}alves, orient. II. Serqueira, Jo\~ao Alves, co-orient}

\notaautorizacao{AUTORIZO A REPRODU\c{C}\~AO E DIVULGA\c{C}\~AO TOTAL OU PARCIAL DESTE TRABALHO, POR QUALQUER MEIO CONVENCIONAL OU ELETR\^ONICO PARA FINS DE ESTUDO E PESQUISA, DESDE QUE CITADA A FONTE.}
%\notabib{Ficha catalogr\'afica revisada pelo Servi\c{c}o de Biblioteca e Informa\c{c}\~ao Prof. Bernhard Gross, com os dados fornecidos pelo(a) autor(a)}

\newcommand{\programa}[1]{

% DFA ==========================================================================
    \ifthenelse{\equal{#1}{DFA}}{
     	\renewcommand{\areaname}{Concentration area:}
			\renewcommand{\opcaoname}{Option:}
			\tipotrabalho{Thesis (Doctor in Science)}
	        \area{Applied Physics}
	       % \opcao{Biomolecular Physics}
	        % O preambulo deve conter o tipo do trabalho, o objetivo, 
			% o nome da institui��o, a �rea de concentra��o e op��o quando houver
			\preambulo{Thesis presented to the Graduate Program in Physics at the Instituto de F\'isica de S\~ao Carlos, Universidade de S\~ao Paulo, to obtain the degree of Doctor in Science.}
			\notaficha{Thesis (Doctorate - Graduate Program in Applied Physics)}
        }{
% MFA ===========================================================================
        \ifthenelse{\equal{#1}{MFA}}{
	        \tipotrabalho{Disserta\c{c}\~ao (Mestrado em Ci\^encias)}
	        \area{F\'isica}
			%\opcao{Nome da Op��o}
	        % O preambulo deve conter o tipo do trabalho, o objetivo, 
			% o nome da institui��o, a �rea de concentra��o e op��o quando houver
			\preambulo{Dissertation presented to the
			Graduate Porgram in Physics at the 
			Instituto de F\'isica de S\~ao Carlos, Universidade de S\~ao Paulo to obtain the degree of Master of Science.}
			\notaficha{Disserta\c{c}\~ao (Mestrado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica Aplicada)}
        }{
% DFAFC ==========================================================================
    \ifthenelse{\equal{#1}{DFAFC}}{
     	\tipotrabalho{Tese (Doutorado em Ci\^encias)}
        \area{F\'isica Aplicada}
        \opcao{F\'isica Computacional}
        % O preambulo deve conter o tipo do trabalho, o objetivo, 
		% o nome da institui��o, a �rea de concentra��o e op��o quando houver
		\preambulo{Tese apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Doutor em Ci\^encias.}
		\notaficha{Tese (Doutorado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica Aplicada)}
    }{
% MFAFC ===========================================================================
        \ifthenelse{\equal{#1}{MFAFC}}{
			\tipotrabalho{Disserta\c{c}\~ao (Mestrado em Ci\^encias)}
	        \area{F\'isica Aplicada}
	        \opcao{F\'isica Computacional}
	        % O preambulo deve conter o tipo do trabalho, o objetivo, 
			% o nome da institui��o, a �rea de concentra��o e op��o quando houver
			\preambulo{Disserta\c{c}\~ao apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Mestre em Ci\^encias.}
			\notaficha{Disserta\c{c}\~ao (Mestrado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica Aplicada)}
        }{
% DFAFBp ===========================================================================
        \ifthenelse{\equal{#1}{DFAFBp}}{
			\tipotrabalho{Tese (Doutorado em Ci\^encias)}
	        \area{F\'isica Aplicada}
	        \opcao{F\'isica Biomolecular}
	        % O preambulo deve conter o tipo do trabalho, o objetivo, 
			% o nome da institui��o, a �rea de concentra��o e op��o quando houver
			\preambulo{Tese apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Doutor em Ci\^encias.}
			\notaficha{Tese (Doutorado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica Aplicada)}
        }{				
% DFAFBe ===========================================================================
        \ifthenelse{\equal{#1}{DFAFBe}}{
			\renewcommand{\areaname}{Concentration area:}
			\renewcommand{\opcaoname}{Option:}
			\tipotrabalho{Thesis (Doctor in Science)}
	        \area{Applied Physics}
	        \opcao{Biomolecular Physics}
	        % O preambulo deve conter o tipo do trabalho, o objetivo, 
			% o nome da institui��o, a �rea de concentra��o e op��o quando houver
			\preambulo{Thesis presented to the Graduate Program in Physics at the Instituto de F\'isica de S\~ao Carlos, Universidade de S\~ao Paulo, to obtain the degree of Doctor in Science.}
			\notaficha{Thesis (Doctorate - Graduate Program in Applied Physics)}
        }{				
% MFAFB ===========================================================================
        \ifthenelse{\equal{#1}{MFAFB}}{
	        \tipotrabalho{Disserta\c{c}\~ao (Mestrado em Ci\^encias)}
	        \area{F\'isica Aplicada}
	        \opcao{F\'isica Biomolecular}
	        % O preambulo deve conter o tipo do trabalho, o objetivo, 
			% o nome da institui��o, a �rea de concentra��o e op��o quando houver
			\preambulo{Disserta\c{c}\~ao apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Mestre em Ci\^encias.}
			\notaficha{Disserta\c{c}\~ao (Mestrado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica Aplicada)}
        }{
				
% DFB ==========================================================================
    \ifthenelse{\equal{#1}{DFB}}{
     	\tipotrabalho{Tese (Doutorado em Ci\^encias)}
        \area{F\'isica B\'asica}
		%\opcao{Nome da Op��o}
        % O preambulo deve conter o tipo do trabalho, o objetivo, 
		% o nome da institui��o, a �rea de concentra��o e op��o quando houver				
		\preambulo{Tese apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Doutor em Ci\^encias.}
		\notaficha{Tese (Doutorado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica B\'asica)}
    }{
% MFB ===========================================================================
        \ifthenelse{\equal{#1}{MFB}}{
        \renewcommand{\areaname}{Concentration area:}
	        \tipotrabalho{Disserta\c{c}\~ao (Mestrado em Ci\^encias)}
	        \area{Theoretical and Experimental Physics}
			%\opcao{Nome da Op��o}
	        % O preambulo deve conter o tipo do trabalho, o objetivo, 
			% o nome da institui��o, a �rea de concentra��o e op��o quando houver				
			\preambulo{Dissertation presented to the
			Graduate Program in Physics at the 
			Instituto de F\'isica de S\~ao Carlos, Universidade de S\~ao Paulo to obtain the degree of Master of Science.}
			\notaficha{Disserta\c{c}\~ao (Mestrado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica B\'asica)}
        }{                
% Outros
				\tipotrabalho{Disserta\c{c}\~ao/Tese (Mestrado/Doutorado)}
				\area{Nome da \'Area}
				\opcao{Nome da Op\c{c}\~ao}
		        % O preambulo deve conter o tipo do trabalho, o objetivo, 
				% o nome da institui��o, a �rea de concentra��o e op��o quando houver
				\preambulo{Disserta\c{c}\~ao/Tese apresentada ao Programa de P\�{\o}s-Gradua\c{c}\~ao em F\�{\i}sica do Instituto de F\�{\i}sica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten�\c{c}\~ao do t\�{\i}tulo de Mestre/Doutor em Ci\^encias.}
				\notaficha{Disserta\c{c}\~ao/Tese (Mestrado/Doutorado - Programa de P\'os-Gradua\c{c}\~ao em Nome da \'Area)}
        }}}}}}}}}}
				
				








==> USPSC-unidades.tex <==
%% USPSC-unidadesTCC.tex
% Camando para definição do programa de Pós-Graduação, Especialidade do Título e Instituição - 21/09/2015
\newcommand{\siglaunidade}[1]{


% EESC-TCC ==========================================================================
    \ifthenelse{\equal{#1}{EESC-TCC}}{
     			\include{USPSC-TCC-pre-textual-EESC}
% ---
    }{
% EESC ==========================================================================
	\ifthenelse{\equal{#1}{EESC}}{
	\include{USPSC-pre-textual-EESC}
	% ---
}{    
% IAU ===========================================================================
        \ifthenelse{\equal{#1}{IAU}}{
        \include{USPSC-pre-textual-IAU}    
        }{
% ICMC ===========================================================================
        \ifthenelse{\equal{#1}{ICMC}}{
        \include{USPSC-pre-textual-ICMC}    
        }{
% IFSC ===========================================================================
        \ifthenelse{\equal{#1}{IFSC}}{
        \include{USPSC-pre-textual-IFSC}    
        }{
% IQSC ===========================================================================
        \ifthenelse{\equal{#1}{IQSC}}{
        \include{USPSC-pre-textual-IQSC}    
        }{

                   
% Outros ========================================================================
                       % ------------------------------------------------------------------------
        \include{USPSC-pre-textual-OUTRO} 
								  }
                }
							}
						}
				}
			}}
         	


==> chap7.tex <==
\chapter{Conclusion}

\label{chap7}

Stochastic thermodynamics is a rich and broad field. In this thesis, we explored some of its subjects using a simulation of a Brownian particle in a harmonic potential. We have begun with a quick presentation of the optical tweezers setup, followed by the Langevin and Fokker-Planck equations. Then, we introduced the concept of stochastic work. Although work fluctuates in each realization, its average value is still larger than the free energy difference of the system. The natural question that arises is what is the optimal protocol. In the overdamped regime, the optimal protocol was already analytically found in the breathing parabola case. Hence, we had a quantifier of the performance of other approximate methods. 

Usually, it is a difficult task to encounter the optimal protocol analytically. Thus we must resort to other approximate methods. 
 We have dealt with two methods from linear response theory, one for slowly varying processes and one phenomenological method. The main result was the numerical verification of the performance of each method for different protocol times and intensities. Besides, we found that the protocols from linear response have good performance even outside its theoretical regime of validity. To verify the reliability of our simulations, we have used the Jarzynski equality and the Crooks relation. Because the Jarzynski equality is an average over exponentials, its convergence can be sensitive to rare events, i.e., the number of realizations can be huge to see the Jarzysnki equality converging. We have discussed the relation between the number of realizations and the protocol time. 

The second topic treated was Maxwell's demon thought experiment, where utilization of fluctuations and information about the state of the particle allows converting information to energy. First, we reproduced some of the results of reference X about the information-to-energy conversion and the generalized Jarzynski equality. To do the information-to-energy conversion in our optical tweezers, we have proposed another experiment, which uses the breathing parabola. This proposal constitutes our second main result.  

The exorcizing of Maxwell's Demon comes from considering Landauer's principle. Thus, we also verified Landauer's principle by simulating the experiment done in reference Y. 

Several paths can be taken from this point. 


\section{Future directions}
\subsection{The underdamped regime}
Several paths can be taken from this point. Throughout this dissertation, we consider that the system was in the overdamped regime in contact with a single thermal reservoir. Therefore, changing to the underdamped regime or adding more heat baths are possible directions for theoretical and experimental studies in the future.  

A topic not yet explored experimentally is the optimal protocols in the underdamped regime. To achieve this limit, modifications in our optical tweezers setup are necessary. By decreasing the friction coefficient and increasing the trap stiffness, and the particle's mass the underdamped regime can be achieved.
  
The friction coefficient can be modified if we consider other medium, with a smaller viscosity, as air. By controlling the laser's intensity, we can increase the trap stiffness. However, this results in very small fluctuations of the particle's position around the trap's center. Thus, precision in the acquisition of the position is necessary.    The mass can be increased if we consider a larger particle. Nonetheless, the particle size affects both the trap stiffness and the friction coefficient. The latter parameter increases with the particle's size, so care must be taken.   


\subsection{More than one heat bath}

The Carnot efficiency was an essential result in the development of classical thermodynamics. Recently, a Brownian Carnot engine was implemented experimentally. To realize thermal machines in our optical tweezers, one of the challenges is to change and control the temperature. Instead of adding heat to the experiment, the idea is to apply a stochastic force that mimics the thermal noise. In ref. \cite{martinez2016brownian}, by using this method, they changed the temperature from room temperature up to thousands of kelvin. 

The capability of changing the temperature allows us to explore other topics as the power output of thermal machines \cite{defaveri2017power} or the role of nonlinearities for the functioning of these machines. \cite{defaveri2018dependence}
